A multiresolution Discrete Element Method for triangulated objects with implicit timestepping

Simulations of many rigid bodies colliding with each other sometimes yield particularly interesting results if the colliding objects differ significantly in size and are non-spherical. The most expensive part within such a simulation code is the collision detection. We propose a family of novel multiscale collision detection algorithms that can be applied to triangulated objects within explicit and implicit time stepping methods. They are well-suited to handle objects that cannot be represented by analytical shapes or assemblies of analytical objects. Inspired by multigrid methods and adaptive mesh refinement, we determine collision points iteratively over a resolution hierarchy, and combine a functional minimisation plus penalty parameters with the actual comparision-based geometric distance calculation. Coarse surrogate geometry representations identify "no collision" scenarios early on and otherwise yield an educated guess which triangle subsets of the next finer level potentially yield collisions. They prune the search tree, and furthermore feed conservative contact force estimates into the iterative solve behind an implicit time stepping. Implicit time stepping and non-analytical shapes often yield prohibitive high compute cost for rigid body simulations. Our approach reduces these cost algorithmically by one to two orders of magnitude. It also exhibits high vectorisation efficiency due to its iterative nature.

==> Results/08a_surrogate-properties-volumes.tex <==
\begin{table}
 \caption{
   Bounding volume of the surrogate model vs.~the real model for the setups from
   Table \ref{table:surrogate-properties:bounding-sphere}.  
   \label{table:surrogate-properties:bounding-sphere-volume}
 }
 \begin{center} 
 {\footnotesize
 \begin{tabular}{|r|rr|rr|rr|}
  \hline
  & \multicolumn{2}{|c|}{$N_{\text{triangles}}=20$}
  & \multicolumn{2}{|c|}{$N_{\text{triangles}}=320$}
  & \multicolumn{2}{|c|}{$N_{\text{triangles}}=1,280$}
  \\
  $\eta _r $ 
  & $\text{V}_{k_{\text{max}}}$
  & $V_{\text{sphere}}$
  & $\text{V}_{k_{\text{max}}}$
  & $V_{\text{sphere}}$
  & $\text{V}_{k_{\text{max}}}$
  & $V_{\text{sphere}}$
  \\
  \hline
  0.0
  & 1.85 & 0.52 & 2.54 & 0.52 & 3.99 & 0.52
  \\
  0.1
  & 2.15 & 0.90 & 2.63 & 0.90 & 2.36 & 0.90
  \\
  0.2
  & 2.51 & 1.44 & 3.00 & 1.44 & 3.28 & 1.44
  \\
  0.4
  & 3.24 & 2.14 & 5.52 & 2.14 & 4.96 & 2.14
  \\
  0.8
  & 4.93 & 3.05 & 8.75 & 3.05 & 10.53 & 3.05
  \\
  \hline
 \end{tabular}
 }
 \end{center}
\end{table}

\begin{table}
 \caption{
   Bounding volume of the surrogate model vs.~the real model for the setups from
   Table \ref{table:surrogate-properties:bounding-sphere} with no N -> N+1 guarantee.  
   \label{table:surrogate-properties:bounding-sphere-volume:fit-fine}
 }
 \begin{center} 
 {\footnotesize
 \begin{tabular}{|r|rr|rr|rr|}
  \hline
  & \multicolumn{2}{|c|}{$N_{\text{triangles}}=20$}
  & \multicolumn{2}{|c|}{$N_{\text{triangles}}=320$}
  & \multicolumn{2}{|c|}{$N_{\text{triangles}}=1,280$}
  \\
  $\eta _r $ 
  & $\text{V}_{k_{\text{max}}h}$
  & $V_{\text{sphere}}$
  & $\text{V}_{k_{\text{max}}h}$
  & $V_{\text{sphere}}$
  & $\text{V}_{k_{\text{max}}h}$
  & $V_{\text{sphere}}$
  \\
  \hline
  0.0
  & 0.84 & 0.52 & 0.63 & 0.52 & 0.70 & 0.52
  \\
  0.1
  & 0.77 & 0.90 & 0.78 & 0.90 & 0.83 & 0.90
  \\
  0.2
  & 1.14 & 1.44 & 0.98 & 1.44 & 1.16 & 1.44
  \\
  0.4
  & 1.55 & 2.14 & 1.71 & 2.14 & 1.58 & 2.14
  \\
  0.8
  & 2.36 & 3.05 & 3.29 & 3.05 & 4.06 & 3.05
  \\
  \hline
 \end{tabular}
 }
 \end{center}
\end{table}


==> Results/08c_hybrid-vs-comparison_backup.tex <==

\begin{table}[ht]
\caption{Particle-particle Comparison}
\centering
\begin{tabular}{| c c c c c c c c c |}
\hline
Triangles & Runtime & AVX SP & SP & Mem bandwidth & Op int & L1-L2 & L2-L3 & L3-system \\
\hline
12 & 0.999 & 0 & 3.57e+03 & 451 & 22.4 & 45.9 & 37.6 & 31.7 \\
36 & 2.08 & 0 & 3.52e+03 & 73.2 & Missing & 24.6 & 9.01 & 9.95 \\
140 & 5.2 & 0 & 3.15e+03 & 30.6 & 186 & 12.5 & 2.82 & 4.32 \\
1224 & 174 & 0 & 3.02e+03 & 26.8 & 185 & 269 & 4.5 & 5.98 \\

\hline
\end{tabular}
\label{Tab:Scenario-bf}
\end{table}

\begin{table}[ht]
\caption{Particle-particle Hybrid}
\centering
\begin{tabular}{| c c c c c c c c c |}
\hline
Triangles & Runtime & AVX SP & SP & Mem bandwidth & Op int & L1-L2 & L2-L3 & L3-system \\
\hline
12 & 0.76 & 1.18e+04 & 1.32e+04 & 1.14e+03 & 20.4 & 306 & 87.5 & 64.4 \\
36 & 1.11 & 1.5e+04 & 1.62e+04 & 114 & Missing & 814 & 45.8 & 23.5 \\
140 & 2.49 & 1.91e+04 & 1.97e+04 & 116 & 326 & 312 & 91.4 & 26.4 \\
1224 & 87.4 & 2e+04 & 2.04e+04 & 1.15e+03 & 21.5 & 150 & 77.9 & 91.3 \\

\hline
\end{tabular}
\label{Tab:Scenario-hybrid}
\end{table}

\begin{table}[ht]
\caption{\replaced[id=Add]{Particle-plane}{Particle-plate} comparison}
\centering
\begin{tabular}{| c c c c c c c c c |}
\hline
Triangles & Runtime & AVX SP & SP & Mem bandwidth & Op int & L1-L2 & L2-L3 & L3-system \\
\hline
12 & 0.000691 & 0 & 3.81e+03 & Missing & Missing & Missing & Missing & Missing \\
36 & 3.26 & 0 & 3.93e+03 & 226 & 126 & 28.3 & 16.8 & 15 \\
140 & 11.2 & 0 & 4.97e+03 & 72.2 & 83.1 & 39.2 & 7.05 & 7.47 \\
1224 & 5.14 & 0 & 4.97e+03 & 32.6 & 410 & 112 & 53.8 & 20.4 \\

\hline
\end{tabular}
\label{Tab:Scenario-bf}
\end{table}

\begin{table}[ht]
\caption{\replaced[id=Add]{Particle-plane}{Particle-plate} hybrid}
\centering
\begin{tabular}{| c c c c c c c c c |}
\hline
Triangles & Runtime & AVX SP & SP & Mem bandwidth & Op int & L1-L2 & L2-L3 & L3-system \\
\hline
36 & 3.29 & 1.23e+04 & 1.37e+04 & 398 & 201 & 217 & 31.5 & 24.7 \\
140 & 11 & 1.36e+04 & 1.51e+04 & 72.4 & 250 & 614 & 22.4 & 15.2 \\
1224 & 19.3 & 1.67e+04 & 1.78e+04 & 57.7 & 263 & 679 & 388 & 116 \\

\hline
\end{tabular}
\label{Tab:Scenario-hybrid}
\end{table}




\begin{table}[htb]
 \caption{
  Particle-particle scenario (top) and particle-on-plane (bottom).
  We compare a comparison-based realisation against a hybrid realisation.
  Per setup, we present the time-to-solution ([t]=s) per Euler step, i.e.~one
  run through all possible triangle combinations,
  and we augment these data with MFlop/s rates split up into scalar and
  vectorised contributions.
  Furthermore, we provide the memory throughput in MB/s. 
  For the hybrid setup, we finally quantiy how many triangle pairs had to be
  checked a posterioi, i.e.~as fallback, by the comparison-based algorithm. 
  This runtime is included in the data.
  \label{table:hybrid-vs-comparison}
 }
 \begin{center}
 \footnotesize
 \begin{tabular}{|r|rrrr|rrrrr|}
\hline
 & \multicolumn{4}{|c|}{Comparison-based}
 & \multicolumn{5}{|c|}{Hybrid} \\
$|N_{\text{triangles}}|$ 
 & Runtime & AVX & Scalar & Mem
 & Runtime & AVX & Scalar & Mem & Fallback
 \\
\hline
12 
 & 0.999 & 0 & 3.57e+03 & 451
 & 0.760 & 1.18e+04 & 1.32e+04 & 1,140 & 7.7\%
 \\
36 
 & 2.08 & 0 & 3.52e+03 & 73.2
 & 1.11 & 1.5e+04 & 1.62e+04 & 114 & 4.5\%
 \\
140 
 & 5.20 & 0 & 3.15e+03 & 30.6
 & 2.49 & 1.91e+04 & 1.97e+04 & 116 & 1.2\%
 \\
1224 
 & 174 & 0 & 3.02e+03 & 26.8
 & 87.4 & 2.00e+04 & 2.04e+04 & 1,150 & 0.028\%
 \\
\hline
12  
 & 6.91e-4 & 0 & 3.81e+03 & xxx
 & xxx & xxx & xxx & xxx & 6.3\%
 \\
36  
 & 3.26 & 0 & 3.93e+03 & 226
 & 3.29 & 1.23e+04 & 1.37e+04 & 398 & 5.1\%
 \\
140  
 & 11.2 & 0 & 4.97e+03 & 72.2
 & 11 & 1.36e+04 & 1.51e+04 & 72.4 & 4.8\%
 \\
1224 
 & 5.14 & 0 & 4.97e+03 & 32.6
 & 19.3 & 1.67e+04 & 1.78e+04 & 57.7 & 3.6\%
 \\
\hline
\end{tabular}
 \end{center}
\end{table}


==> a1_direct-detection.tex <==
\appendix


\section{Surrogate triangle gradient descent}
\label{section:appendix:surrogate_gradient}

\subsection*{Maxima script common components:}

dotv(A,B):=dot(A[1],A[2],A[3],B[1],B[2],B[3]);

gradef(dot(a,b,c,d,e,f),d,e,f,a,b,c);

dot2(A) := dotv(A,A);

X(P) := [P[1], P[2], P[3]];

A(P) := [P[4], P[5],P[6]];

B(P) := [P[7],P[8],P[9]];

C(P) := [P[10],P[11],P[12]];

AX(P) := X(P)-A(P);

AB(P):=B(P)-A(P);

AC(P):=C(P)-A(P);

N(P):=crossv(AB(P),AC(P));

D(P):=dotv(N(P),A(P));

a00(P) := dot2(AB(P));

a01(P):=dotv(AB(P),AC(P));

a11(P):=dot2(AC(P));

b0(P):=-dotv(AX(P),AB(P));

b1(P):=-dotv(AX(P), AC(P));

det(P):=a00(P)*a11(P)-a01(P)*a01(P);


\subsection*{Select one of these by uncommenting one.  Defines the closest point on the triangle as barycentric coordinates (t0 and t1):}

V0
 
/*t0(P):=0; t1(P):=0;*/

V1
 
/*t1(P) :=0; t0(P):=1;*/

V2
 
/*t0(P):=0; t1(P):=1;*/

E01
 
/*t0(P):=1; t0(P):=-b0(P)/a00(P);*/

E20
 
/*t0(P):=0; t1(P):=-b1(P)/a11(P);*/

E12
 
/*t0(P):=(a11(P)+b1(P)-(a01(P)+b0(P)))/(a00(P)-2*a01(P)+a11(P));
	t1(P):=1-t0(P);*/

 Region 0
 
/*dist(P):=(dotv(N(P),X(P))-D(P)) / sqrt(dotv(N(P),N(P)));

dist2(P):=dist(P)*dist(P);*/

\subsection*{Turn barycentric coordinates to distance function.  (Comment out if using Region 0):}

closest(P):=A(P)+t0(P)*AB(P)+t1(P)*AC(P);

di(P):=X(P)-closest(P);

dist2(P):=dot2(di(P));

\subsection*{Compute gradient:}

diff(dist2([x,y,z,a,b,c,d,e,f,g,h,i]),a);

diff(dist2([x,y,z,a,b,c,d,e,f,g,h,i]),b);

diff(dist2([x,y,z,a,b,c,d,e,f,g,h,i]),c);

diff(dist2([x,y,z,a,b,c,d,e,f,g,h,i]),d);

diff(dist2([x,y,z,a,b,c,d,e,f,g,h,i]),e);

diff(dist2([x,y,z,a,b,c,d,e,f,g,h,i]),f);

diff(dist2([x,y,z,a,b,c,d,e,f,g,h,i]),g);

diff(dist2([x,y,z,a,b,c,d,e,f,g,h,i]),h);

diff(dist2([x,y,z,a,b,c,d,e,f,g,h,i]),i);

\subsection*{Code to choose which gradient function to use for a point X and triangle (A, B, C):}

\begin{lstlisting}[language=C++]
gradient point_gradient(const vec3 X,
    const vec3 A,
    const vec3 B,
    const vec3 C)
{
    vec3 AX = sub(X, A);
    vec3 AB= sub(B, A);
    vec3 AC = sub(C, A);
    float a00 = DOT(AB, AB);
    float a01 = DOT(AB, AC);
    float a11 = DOT(AC, AC);
    float b0 = -DOT(AX, AB);
    float b1 = -DOT(AX, AC);
    float det = a00 * a11 - a01 * a01;
    float t0 = a01 * b1 - a11 * b0;
    float t1 = a01 * b0 - a00 * b1;

    if (t0 + t1 <= det) {
        if (t0 < 0.0) {
            if (t1 < 0.0) {  // region 4
                if (b0 < 0.0) {
                    if (-b0 >= a00) {  // V1
                        return V1(X, A, B, C);
                    } else {  // E01
                        return E01(X, A, B, C);
                    }
                } else {
                    if (b1 >= 0.0) {  // V0
                        return V0(X, A, B, C);
                    } else if (-b1 >= a11) {  // V2
                        return V2(X, A, B, C);
                    } else {  // E20
                        return E20(X, A, B, C);
                    }
                }
            } else {  // region 3
                if (b1 >= 0.0) {  // V0
                    return V0(X, A, B, C);
                } else if (-b1 >= a11) {  // V2
                    return V2(X, A, B, C);
                } else {  // E20
                    return E20(X, A, B, C);
                }
            }
        } else if (t1 < 0.0) {  // region 5
            if (b0 >= 0.0) { // V0
                return V0(X, A, B, C);
            } else if (-b0 >= a00) {  // V1
                return V1(X, A, B, C);
            } else {  // E01
                return E01(X, A, B, C);
            }
        } else {  // region 0, interior
            return region0(X, A, B, C);
        }
    } else {
        if (t0 < 0.0) {  // region 2
            float tmp0 = a01 + b0;
            float tmp1 = a11 + b1;
            if (tmp1 > tmp0) {
                float numer = tmp1 - tmp0;
                float denom = a00 - 2*a01 + a11;
                if (numer >= denom) {  // V1
                    return V1(X, A, B, C);
                } else {  // E12
                    return E12(X, A, B, C);
                }
            } else {
                if (tmp1 <= 0.0) {  // V2
                    return V2(X, A, B, C);
                } else if (b1 >= 0.0) {  // V0
                    return V0(X, A, B, C);
                } else {  // E20
                    return E20(X, A, B, C);
                }
            }
        } else if (t1 < 0.0) {  // region 6
            float tmp0 = a01 + b1;
            float tmp1 = a00 + b0;
            if (tmp1 > tmp0) {
                float numer = tmp1 - tmp0;
                float denom = a00 - 2*a01 + a11;
                if (numer >= denom) {  // V2
                    return V2(X, A, B, C);
                } else {  // E12
                    return E12(X, A, B, C);
                }
            } else {
                if (tmp1 <= 0.0) {  // V1
                    return V1(X, A, B, C);
                } else if (b0 >= 0.0) {  // V0
                    return V0(X, A, B, C);
                } else {  // E01
                    return E01(X, A, B, C);
                }
            }
        } else {  // region 1
            float numer = a11 + b1 - a01 - b0;
            if (numer <= 0.0) {  // V2
                return V2(X, A, B, C);
            } else {
                float denom = a00 - 2*a01 + a11;
                if (numer >= denom) {  // V1
                    return V1(X, A, B, C);
                } else {  // E12
                    return E12(X, A, B, C);
                }
            }
        }
    }
}
\end{lstlisting}

==> a3_iterative-contact-detection.tex <==
\section{Iterative contact detection}


Let the points $x_A$ and $x_B$ be points on two triangles $A$ and $B$ that are parameterised through their barycentric coordinate system:
\begin{eqnarray*}
 x_A & = & a (x_{A,2}-x_{A,1}) + b (x_{A,3}-x_{A,1})  
   \qquad 0 \leq a,b \leq 1
   \\
 x_B & = & c (x_{B,2}-x_{B,1}) + d (x_{B,3}-x_{B,1})
   \qquad 0 \leq c,d \leq 1.
\end{eqnarray*}

\noindent
The points $x_{A,1}, x_{A,2}, x_{A,3}$ are the vertices of the triangle $A$,
$x_{B,1}, x_{B,2}, x_{B,3}$ the vertices of $B$.
We are interested in $\min _{a,b,c,d} \| x_A - x_B \|_2$, but instead compute
\[
  \min _{a,b,c,d} \frac{1}{2} \| x_A - x_B \|_2^2.
\]

\noindent
The power two eliminates an expensive square root, and it ensures that the 
minimum function does not have a sharp kink but instead is a smooth parabula, i.e.~has a derivative everywhere.
Still, this baseline function lacks the fact that the coordinates are bounded by 0 and 1, 
and the parabula can degenerate into a line without a unique minimum if two triangles are parallel.
In this case, there is no unique closest point pair on the triangle.
We add the range of the barycentric coordinates via a penalty term, i.e.~we enforce it weakly:
\[
  \min _{a,b,c,d} 
  \underbrace{
  \frac{1}{2} \| x_A - x_B \|_2^2 + \alpha \left( \max(0,-a) + \max(0,-b) + \ldots \max(0,a-1) + \ldots \right)
  }_{=: J(a,b,c,d)}.
\]

\noindent
As $J(a,b,c,d)$ is convex, we are effectively searching for 
\[
\nabla_{a,b,c,d} J(a,b,c,d) = 0.
\]

\noindent
As $J(a,b,c,d)$ is non-linear we solve it via Newton.
As $J(a,b,c,d)$ is not smooth around the $\max $, and as the problem is ill-posed for (close to) parallel triangles, 
it is not reasonable to work with the Hessian $\nabla_{a,b,c,d} \nabla_{a,b,c,d} J(a,b,c,d)$.
Instead, we work with its diagonal, and we add a helper diagonal to the inverse, to accommodate the ill-posedness.
Therfore, 
\[
 (a,b,c,d)^{(n+1)} = 
 (a,b,c,d)^{(n)} -
 \left(
 \underbrace{
 \nabla_{a,b,c,d} \nabla_{a,b,c,d} J(a,b,c,d)^{(n)} + \epsilon \ id
 }_{\text{Hessian plus }\epsilon}
 \right)^{-1}
\nabla_{a,b,c,d} J(a,b,c,d)^{(n)} 
\]

\noindent
becomes
\begin{eqnarray*}
 \left(
  \begin{array}{c} a \\ b \\ c \\ d \end{array}
 \right)^{(n+1)}
 & = &
 \left(
  \begin{array}{c} a \\ b \\ c \\ d \end{array}
 \right)^{(n)}
 \\
 & - &
 \left(
  \begin{array}{cccc} 
    \frac{1}{\epsilon + \partial _a \partial _a J(a,b,c,d)^{(n)}} & 0 & 0 & 0 \\ 
    0 & \frac{1}{\epsilon + \partial _b \partial _b J(a,b,c,d)^{(n)}} & 0 & 0 \\ 
    0 & 0 & \frac{1}{\epsilon + \partial _c \partial _c J(a,b,c,d)^{(n)}} & 0  \\ 
    0 & 0 & 0 & \frac{1}{\epsilon + \partial _d \partial _d J(a,b,c,d)^{(n)}} 
  \end{array}
 \right) \\
 &&
 \left(
  \begin{array}{c} 
    \partial _a J(a,b,c,d)^{(n)} \\ 
    \partial _b J(a,b,c,d)^{(n)} \\ 
    \partial _c J(a,b,c,d)^{(n)} \\ 
    \partial _d J(a,b,c,d)^{(n)} 
  \end{array}
 \right).
\end{eqnarray*}

\noindent
where $a^{(0)}=b^{(0)}=c^{(0)}=d^{(0)} \approx \frac{1}{3}$ and $\epsilon >0 $ is a fixed, small constant.
We let 
\[
\theta(x) = \left\{
  \begin{array}{rl}
   1 & x\geq0 \\
   0 & x<0
  \end{array}
\right.
\]

\noindent
denote the heaviside function and end up with the update rules
\begin{eqnarray*}
a & \gets &
a - \frac{1.0 \left(- \alpha \theta\left(- a\right) + \alpha \theta\left(a - 1\right) + \left(x_{a11} - x_{a21}\right) \left(a \left(x_{a11} - x_{a21}\right) + b \left(x_{a11} - x_{a31}\right) - c \left(x_{b11} - x_{b21}\right) - d \left(x_{b11} - x_{b31}\right)\right) + \left(x_{a12} - x_{a22}\right) \left(a \left(x_{a12} - x_{a22}\right) + b \left(x_{a12} - x_{a32}\right) - c \left(x_{b12} - x_{b22}\right) - d \left(x_{b12} - x_{b32}\right)\right) + \left(x_{a13} - x_{a23}\right) \left(a \left(x_{a13} - x_{a23}\right) + b \left(x_{a13} - x_{a33}\right) - c \left(x_{b13} - x_{b23}\right) - d \left(x_{b13} - x_{b33}\right)\right)\right)}{\alpha \delta\left(a\right) + \alpha \delta\left(a - 1\right) + \epsilon + \left(x_{a11} - x_{a21}\right)^{2} + \left(x_{a12} - x_{a22}\right)^{2} + \left(x_{a13} - x_{a23}\right)^{2}}
\\
b & \gets &
b - \frac{1.0 \left(- \alpha \theta\left(- b\right) + \alpha \theta\left(b - 1\right) + \left(x_{a11} - x_{a31}\right) \left(a \left(x_{a11} - x_{a21}\right) + b \left(x_{a11} - x_{a31}\right) - c \left(x_{b11} - x_{b21}\right) - d \left(x_{b11} - x_{b31}\right)\right) + \left(x_{a12} - x_{a32}\right) \left(a \left(x_{a12} - x_{a22}\right) + b \left(x_{a12} - x_{a32}\right) - c \left(x_{b12} - x_{b22}\right) - d \left(x_{b12} - x_{b32}\right)\right) + \left(x_{a13} - x_{a33}\right) \left(a \left(x_{a13} - x_{a23}\right) + b \left(x_{a13} - x_{a33}\right) - c \left(x_{b13} - x_{b23}\right) - d \left(x_{b13} - x_{b33}\right)\right)\right)}{\alpha \delta\left(b\right) + \alpha \delta\left(b - 1\right) + \epsilon + \left(x_{a11} - x_{a31}\right)^{2} + \left(x_{a12} - x_{a32}\right)^{2} + \left(x_{a13} - x_{a33}\right)^{2}}
\\
c & \gets &
c - \frac{1.0 \left(- \alpha \theta\left(- c\right) + \alpha \theta\left(c - 1\right) - 1.0 \left(x_{b11} - x_{b21}\right) \left(a \left(x_{a11} - x_{a21}\right) + b \left(x_{a11} - x_{a31}\right) - c \left(x_{b11} - x_{b21}\right) - d \left(x_{b11} - x_{b31}\right)\right) - 1.0 \left(x_{b12} - x_{b22}\right) \left(a \left(x_{a12} - x_{a22}\right) + b \left(x_{a12} - x_{a32}\right) - c \left(x_{b12} - x_{b22}\right) - d \left(x_{b12} - x_{b32}\right)\right) - 1.0 \left(x_{b13} - x_{b23}\right) \left(a \left(x_{a13} - x_{a23}\right) + b \left(x_{a13} - x_{a33}\right) - c \left(x_{b13} - x_{b23}\right) - d \left(x_{b13} - x_{b33}\right)\right)\right)}{\alpha \delta\left(c\right) + \alpha \delta\left(c - 1\right) + \epsilon + 1.0 \left(x_{b11} - x_{b21}\right)^{2} + 1.0 \left(x_{b12} - x_{b22}\right)^{2} + 1.0 \left(x_{b13} - x_{b23}\right)^{2}}
\\
d & \gets &
d - \frac{1.0 \left(- \alpha \theta\left(- d\right) + \alpha \theta\left(d - 1\right) - 1.0 \left(x_{b11} - x_{b31}\right) \left(a \left(x_{a11} - x_{a21}\right) + b \left(x_{a11} - x_{a31}\right) - c \left(x_{b11} - x_{b21}\right) - d \left(x_{b11} - x_{b31}\right)\right) - 1.0 \left(x_{b12} - x_{b32}\right) \left(a \left(x_{a12} - x_{a22}\right) + b \left(x_{a12} - x_{a32}\right) - c \left(x_{b12} - x_{b22}\right) - d \left(x_{b12} - x_{b32}\right)\right) - 1.0 \left(x_{b13} - x_{b33}\right) \left(a \left(x_{a13} - x_{a23}\right) + b \left(x_{a13} - x_{a33}\right) - c \left(x_{b13} - x_{b23}\right) - d \left(x_{b13} - x_{b33}\right)\right)\right)}{\alpha \delta\left(d\right) + \alpha \delta\left(d - 1\right) + \epsilon + 1.0 \left(x_{b11} - x_{b31}\right)^{2} + 1.0 \left(x_{b12} - x_{b32}\right)^{2} + 1.0 \left(x_{b13} - x_{b33}\right)^{2}}
\end{eqnarray*}


\noindent
where $\delta $ is the delta function, i.e.~equals 1 if and only if the arguments equals 0.
This heaviside function kicks in whenever the weak admissibility penalties become active.
In the implementation, it is reasonable to set $\delta (x)=0$ via a lambda expression. 
We obtain a code fragment similar to 
\begin{verbatim}
auto Square(double x)->double {return x*x;}
auto Heaviside(double x)->double {return x<0 ? 0.0 : 1.0;}
a = a - 1.0*(-\alpha*Heaviside(-a) + \alpha*Heaviside(a - 1) + (x_a11 - x_a21)*(a*(x_a11 - x_a21) + b*(x_a11 - x_a31) - c*(x_b11 - x_b21) - d*(x_b11 - x_b31)) + (x_a12 - x_a22)*(a*(x_a12 - x_a22) + b*(x_a12 - x_a32) - c*(x_b12 - x_b22) - d*(x_b12 - x_b32)) + (x_a13 - x_a23)*(a*(x_a13 - x_a23) + b*(x_a13 - x_a33) - c*(x_b13 - x_b23) - d*(x_b13 - x_b33)))/(0*(a) + 0*(a - 1) + \epsilon + Square(x_a11 - x_a21) + Square(x_a12 - x_a22) + Square(x_a13 - x_a23));
b = b - 1.0*(-\alpha*Heaviside(-b) + \alpha*Heaviside(b - 1) + (x_a11 - x_a31)*(a*(x_a11 - x_a21) + b*(x_a11 - x_a31) - c*(x_b11 - x_b21) - d*(x_b11 - x_b31)) + (x_a12 - x_a32)*(a*(x_a12 - x_a22) + b*(x_a12 - x_a32) - c*(x_b12 - x_b22) - d*(x_b12 - x_b32)) + (x_a13 - x_a33)*(a*(x_a13 - x_a23) + b*(x_a13 - x_a33) - c*(x_b13 - x_b23) - d*(x_b13 - x_b33)))/(0*(b) + 0*(b - 1) + \epsilon + Square(x_a11 - x_a31) + Square(x_a12 - x_a32) + Square(x_a13 - x_a33));
c = c - 1.0*(-\alpha*Heaviside(-c) + \alpha*Heaviside(c - 1) - 1.0*(x_b11 - x_b21)*(a*(x_a11 - x_a21) + b*(x_a11 - x_a31) - c*(x_b11 - x_b21) - d*(x_b11 - x_b31)) - 1.0*(x_b12 - x_b22)*(a*(x_a12 - x_a22) + b*(x_a12 - x_a32) - c*(x_b12 - x_b22) - d*(x_b12 - x_b32)) - 1.0*(x_b13 - x_b23)*(a*(x_a13 - x_a23) + b*(x_a13 - x_a33) - c*(x_b13 - x_b23) - d*(x_b13 - x_b33)))/(0*(c) + 0*(c - 1) + \epsilon + 1.0*Square(x_b11 - x_b21) + 1.0*Square(x_b12 - x_b22) + 1.0*Square(x_b13 - x_b23));
d = d - 1.0*(-\alpha*Heaviside(-d) + \alpha*Heaviside(d - 1) - 1.0*(x_b11 - x_b31)*(a*(x_a11 - x_a21) + b*(x_a11 - x_a31) - c*(x_b11 - x_b21) - d*(x_b11 - x_b31)) - 1.0*(x_b12 - x_b32)*(a*(x_a12 - x_a22) + b*(x_a12 - x_a32) - c*(x_b12 - x_b22) - d*(x_b12 - x_b32)) - 1.0*(x_b13 - x_b33)*(a*(x_a13 - x_a23) + b*(x_a13 - x_a33) - c*(x_b13 - x_b23) - d*(x_b13 - x_b33)))/(0*(d) + 0*(d - 1) + \epsilon + 1.0*Square(x_b11 - x_b31) + 1.0*Square(x_b12 - x_b32) + 1.0*Square(x_b13 - x_b33));
\end{verbatim}

==> b8a_surrogate-properties.tex <==
\section{Surrogate model properties}

The bounding volume ratios of our surrogate models compared to the real
geometry's bounding sphere volume are rather high with our current surrogate
model construction algorithm (Table
\ref{table:surrogate-properties:bounding-sphere-volume}).





==> old-text.tex <==
\begin{eqnarray}
\argmin_{x_1,x_2,x_3} && \left(
  \frac{1}{2} | \frac{1}{\frac{1}{4}(x_2-x_1) \times (x_3-x_1)} |^2 + \alpha_1 C
  \right) + \alpha_2 S
 \label{equation:surrogate-triangle-area}
 \\
& = & \argmin_{x_1,x_2,x_3} \Big( \ldots + \alpha_1 \max_{v \in V(\mathbb{T}_h)} \frac{1}{2}|\textit{Pt2T}(v, x_1, x_2, x_3)|^2 \Big) + \alpha_2 S 
 \label{equation:surrogate-triangle-dist}
 \\
& = & \ldots + \alpha_2 N(x_1, x_2, x_3) \min_{v \in V(\mathbb{T}_h)} \textit{Pt2P}(v, x_1, x_2, x_3)
 \label{equation:surrogate-triangle-surface}
\end{eqnarray}

where \textit{Pt2T} is the distance between a point and a triangle and \textit{Pt2P} is the signed distance between a point and a plane.
Where $N(t)$ is the normalised normal vector of triangle $t$.

The minimisation has three terms.
First, (\ref{equation:surrogate-triangle-area}) maximises the area of the surrogate triangle and as a result will be indirectly minimising the distance from the surrogate to each child triangle.
Second, (\ref{equation:surrogate-triangle-dist}) minimises the maximum distance from the surrogate to the child triangles.
The final term (\ref{equation:surrogate-triangle-surface}) moves the surrogate along it's normal direction so that the surrogate is below the surface of the fine resolution geometry.  This final term is only applied--by selecting $\alpha_2$ to be $0$ or $1$--when the surrogate is considered a good representation of the surface.

A Surrogate triangle also has parameters $\mathcal{E}$ and $\epsilon$ which makes it a volumetric object.
These parameters result from the current choice of the surrogate triangle coordinates.
$\mathcal{E}$ is given by the minimum distance to the surrogate triangle over the input triangles.
$\epsilon$ is given once a surrogate tree is constructed by the maximum distance from the surrogate triangle to a child surrogate triangle plus the child surrogate's $\epsilon$.


We intentionally leave the definition of a ``good representation" ambiguous as a variety of heuristics could be applied here.
For our implementation we say it's a ``good representation" of the surface if $\forall t_i \in \mathbb{T}_h, N(t_h) \cdot \textit{Normal}(t_i) > 0$.

Though (\ref{equation:surrogate-triangle-area}-\ref{equation:surrogate-triangle-surface}) is a quadratic cost function, its solution is neither unique nor can it be computed directly.
As we intend to use our surrogate models as helper data structures in 
some phases of the algorithm, we are satisfied with an approximate solution to
(\ref{equation:surrogate-triangle-area}-\ref{equation:surrogate-triangle-surface}) as long as it is consistent.



% 
% todo Ich
%
$|\mathbb{T}^{\epsilon _{(k-1)h}}_{(k-1)h}|>1$ is prescribed.
The surrogate triangle thus trivially is efficient for the input set.
\marginpar{Maybe a separate discussion of the properties?}



% \textsc{MinBound}(\mathbb{G}) computes an [insert name for triangle-epsilon volume] that satisfies the following constraints:
% \[
% t, \mathbb{G}: \argmin_{t^{\testtt{tri}}} \sum_{t_i}^{\mathbb{G}}\Call{RequiredBound}{t, t_i} + \alpha \cdot \Call{Area}{t^{\texttt{tri}}}
% \]
% \[
% \forall t_i \in \mathbb{G}: V(t_i) \subseteq V(t)
% \]

%\textsc{RequiredBound}($t$, $t_i$) computes the minimum epsilon for [insert
% name] t such that $V(t_i) \subseteq V(t)$.  This can be computed directly.




==> simple-multi-resolution-explicit-Euler.tex <==

\section{Poster resources}

\begin{algorithm}[htb]
  \caption{
    Multiresolution explicit time stepping.
    }
  \begin{algorithmic}[1]
  \State $\textsc{S} \textit{: The current state of simulation}$
    \State $C \gets \emptyset$
    \For{$R \in \textsc{Resolutions}$}
        \State $C \gets \textsc{contacts}(S, R, C)$
    \EndFor
    \State $S \gets S + \textsc{state\_change}(C)$

  \end{algorithmic}
\end{algorithm}

\begin{algorithm}[htb]
  \caption{
    Multiresolution Piccard implicit time stepping.
    }
  \begin{algorithmic}[1]
    \State $\textsc{S} \textit{: The current state of simulation}$
    \State $\textsc{P} \textit{: The current prediction of the state update}$
    \While{$\Delta P > \epsilon$}
        \State $C \gets \emptyset$
        \For{$R \in \textsc{Resolutions}$}
            \State $C \gets \textsc{contacts}(S + P, R, C)$
        \EndFor
        \State $P \gets \textsc{state\_change}(C)$
    \EndWhile
    \State $S \gets S + \textsc{state\_change}(C)$

  \end{algorithmic}
\end{algorithm}

\begin{algorithm}[htb]
  \caption{
    Multiresolution Piccard implicit time stepping with inverted loops.
    }
  \begin{algorithmic}[1]
    \State $C \gets \emptyset$
    \State $\textsc{S} \textit{: The current state of simulation}$
    \State $\textsc{P} \textit{: The current prediction of the state update}$
    \For{$R \in \textsc{Resolutions}$}
        \While{$\Delta P > \epsilon$}
            \State $C \gets \textsc{contacts}(S + P, R, C)$
            \State $P \gets \textsc{state\_change}(C)$
        \EndWhile
    \EndFor
    \State $S \gets S + P$
  \end{algorithmic}
\end{algorithm}

\begin{table}[ht]
\caption{Scenario s4}
\centering
\begin{tabular}{| c c c c |}
\hline
Scenario  & Full Runtime [s] & Full Hybrid Runtime [s] & Hierarchy Hybrid Runtime [s] \\
\hline
Particle-particle & 1e+03 & 718 & 2.98 \\
Particle-on-plane & 485 & 336 & 14.6 \\
Hopper & 2.73e+04 & 1.88e+04 & 126 \\

\hline
\end{tabular}
\end{table}

\begin{table}[ht]
\caption{Scenario s4}
\centering
\begin{tabular}{| c c c c c c c |}
\hline
Scenario  & L1-L2 Full & L1-L2 ours & L2-L3 Full & L2-L3 ours & L3-system Full & L3-system ours \\
\hline
Particle-particle & 410 & 101 & 9.29 & 27.1 & 11.6 & 13.8 \\
Particle-on-plane & 186 & 24.2 & 1.14 & 4.75 & 3.52 & 2.51 \\
Hopper & 1.01e+04 & 300 & 63 & 61.5 & 94 & 28.1 \\

\hline
\end{tabular}
\end{table}

$\forall P : \textsc{contact}(P, child) \rightarrow \textsc{contact}(P, parent^\epsilon)$

$\forall P : \textsc{contact}(P, parent^E) \rightarrow \textsc{contact}(P, child)$
